An Intra-BRNN and GB-RVQ Based END-TO-END Neural Audio Codec

Recently, neural networks have proven to be effective in performing speech coding task at low bitrates. However, under-utilization of intra-frame correlations and the error of quantizer specifically degrade the reconstructed audio quality. To improve the coding quality, we present an end-to-end neural speech codec, namely CBRC (Convolutional and Bidirectional Recurrent neural Codec). An interleaved structure using 1D-CNN and Intra-BRNN is designed to exploit the intra-frame correlations more efficiently. Furthermore, Group-wise and Beam-search Residual Vector Quantizer (GB-RVQ) is used to reduce the quantization noise. CBRC encodes audio every 20ms with no additional latency, which is suitable for real-time communication. Experimental results demonstrate the superiority of the proposed codec when comparing CBRC at 3kbps with Opus at 12kbps.

==> sections/architecture_xulinping.tex <==
CBRC encodes a single channel 20ms waveform $x \in \mathbb{R}^{T}$ of duration T samepled at 16kHz. This model consists of an encoder, a quantizer and a decoder, as illustrated in Figure \ref{cbrc_codec}. The codec is trained end-to-end with discriminator and adversarial loss to improve the perceptual quality of the reconstructed audio.
  
% -------------------------------------------------------------------------
% cbrc_codec
\begin{figure}[t]
  \begin{minipage}[b]{1.0\linewidth}
    \centering
    \centerline{\includegraphics[width=0.9\linewidth,height=0.45\linewidth]{pics/codec_structure.png}}
  %  \vspace{2.0cm}
  \end{minipage}
  \caption{
    CBRC model architecture 
  }
  \label{cbrc_codec}
  \vspace{-0.2cm}
  \end{figure}
% -------------------------------------------------------------------------


\subsection{Encoder and decoder}
The encoder adopts four cascaded CBRNBlocks to perform the feature extraction. Each CBRNBlock is composed of three ResidualUnits for extracting features and a Conv1D layer with stride for down-sampling. Same as SoundStream \cite{soundstream}, the number of channels is doubled after down-sampling. A causal 1D convolution layer after four CBRNBlocks sets the dimensionality of  embeddings to $D$=256. To encode an audio waveform at 16kHz, the model configs the stride of the CBRNBlocks to be (2,4,4,5) and encoder computes every $M$=160 samples as one embedding. Thus, the encoder outputs enc($x$)$\in \mathbb{R}^{S \times D}$, with $S = T/M$ is the number of embeddings. The decoder mirrors the encoder, using a transposed convolution for up-sampling. 

Figure \ref{encoder} illustrates the architecture of the CBRNBlock. Each ResidualUnit stacks dilated causal 1D-CNN and Intra-BRNN to form an interleaved structure. The dilation rates in each block are set to (1,3,9).  
An internal buffer is inlcuded in each convolution to use information from past frames in inference mode. Intra-BRNN which consists of Bi-GRU, followed by a linear fully-connected layer and a batchnorm layer, is adopted to capture the intra-frame correlations in each frame.   
% -------------------------------------------------------------------------
% encoder
\begin{figure}[t]
  \begin{minipage}[b]{1.0\linewidth}
    \centering
    \centerline{\includegraphics[width=1\linewidth]{pics/encoder.png}}
  %  \vspace{2.0cm}
  \end{minipage}
  \caption{
    CBRNBlock diagram  
  }
  \label{encoder}
  \vspace{-0.2cm}
  \end{figure}
% -------------------------------------------------------------------------


\subsection{Group-wise RVQ}
The goal of the quantizer is to compress the output of the encoder enc($x$) to a target bitrate $R$, expressed in bits/second (bps). A codeword is selected from $N$ vectors in vector quantizer to encode embeddings of enc($x$). Each embedding is then mapped to a sequence of one-hot vectors of shape $(S, N)$ , which can be represented using $Slog_{2}N$ bits. However, when target bitrate $R$=6kbps, the codebook size of one-shot VQ is huge and computation complexity is also very high \cite{soundstream}.

Residual Vector Quantizer (RVQ) \cite{soundstream} cascades several VQ layers to reduce the codebook size. When target bitrate $R$=6kbps, the number of VQ layers $N_q$=6 and the number of embeddings per second $S$=100, the codebook size of each quantizer $N$=$2^{R/N_{q}/S}$=$2^{10}$=1024, which requires storing a codebook with 6 $\times$ 1024 vectors.
Inputs for each layer of RVQ are the quantization residual from the previous layer. 

A more promising method, named Group-wise RVQ is M adopted. Figure \ref{g_rvq} shows the architecture of the Group-wise RVQ. Group-wise RVQ splits the $D$-dimensional embedding into $G$ sub-groups ($G$ is set to 2 in figure \ref{g_rvq}), and quantizes each sub-group independently. Thus, each sub-group uses a smaller $D/G$-dimmensional codebook and quantizes the split embeding independently. Afterwards, two parallel optimal codewords from sub-groups are concatenated to form the final quantization result.

The number of parameters in RVQ codebook are $N_q \times D \times N$ and the computational complexity of RVQ is $N_q \times (D+1) \times N \times S$ Macs. When $R$=6kbps, $N_q$=6 and  $S$=100, the number of parameters is 1.5M and the complexity of quantization is 0.157G Macs. 
While the Group-wise RVQ uses 2 parallel RVQs with $N_q$=3, 0.79M parameters and 0.079G Macs quantization complexity. Furthermore, the Group-wise RVQ with half parameters and complexity outperforms the typical RVQ by VISQOL score 0.11(see Section 3.4).  

% -------------------------------------------------------------------------
% g_rvq
\begin{figure}[t]
  \begin{minipage}[b]{1.0\linewidth}
    \centering
    \centerline{\includegraphics[width=\linewidth,height=0.55\linewidth]{pics/g_rvq.png}}
  %  \vspace{2.0cm}
  \end{minipage}
  \caption{ Group-wise RVQ: The encoded embedding is split into two independent embeddings. They are parallel in the process of the individual quantization. }
  \label{g_rvq}
  % \vspace{-0.4cm}
\end{figure}
% -------------------------------------------------------------------------


\subsection{Beam-search RVQ}
Besides Group-wise RVQ, we also use Beam-search algorithm to select vectors in larger search space, which futher reduces the quantization error.

% -------------------------------------------------------------------------
% bs-rvq
\begin{figure}[t]
  \begin{minipage}[b]{1.0\linewidth}
    \centering
    \centerline{\includegraphics[width=0.8\linewidth,height=0.42\linewidth]{pics/bs_rvq.png}}
  %  \vspace{2.0cm}
  \end{minipage}
  \caption{Beam-search RVQ: The figure shows the process of quantization path in three layers of VQ when the number of candidates $k$ = 2. Each layer of VQ except the last reserves 2 quantization paths.  
  }
  \label{bs_rvq}
  \vspace{-0.3cm}
  \end{figure}
% -------------------------------------------------------------------------

Algorithm \ref{beam-search} shows Beam-search implementation details. As can be seen, Beam-search RVQ selects vectors based on the minimum quantization path error which is measured by the MSE between the sum of selected vectors and the input embedding. Each VQ layer quantizes the potential $k$ candidates and thus leads to $k^{2}$ new options. After that, among the  $k^{2}$ options, $k$ optional paths with the smallest error are selected as optimal output of the currnet VQ layer. Finally, the best choice among the $k$ potential paths is decided in the last VQ layer. Figure \ref{bs_rvq} shows an example when $k$ is set to 2. Naturally, a larger $k$ in Beam-search RVQ results in a smaller quantization error because the quantization path is selected in larger search space.

Beam-search RVQ slightly increases complexity of the quantization. The computational complexity increases by about $\frac{1+k(N_{q}-1)}{N_{q}}$ times if Beam-search RVQ consists of $N_q$ layers of VQ and $k$ candidates are selected. 


% -------------------------------------------------------------------------
% bs rvq algorithm
\begin{algorithm}[t] 
  \caption{Beam-search RVQ}
  \LinesNumbered 
  \label{beam-search}
  \KwIn{
    Embedding X; Number of candidates k; 
    Vector Quantizers $Q_{i} $  for i = 1 ... $N_{q}$, where $\left[ z_{1}, ... , z_{k}\right] = Q_{i}(residual)$;
  $Res_{topk}= \left[ r_{1}, ... , r_{k}\right]$ where $r_{i}=X$;
  $\left[s_{1}, ..., s_{k}\right] = find(Candidates, k)$ where pick the k values with the smallest value }
  \KwOut{Quantized output Y}
  \For{i= 1 to $N_q$}{
    $Res\_tmp=\left[ \quad \right]$\;
    \For{j = 1 to k}{
      $r = Res_{topk}\left[j\right]$\;
      $\left[ z_{1}, ... ,z_{k}\right] = Q_{i}(r)$\;
      $\left[ r_{1}, ... ,r_{k}\right] = \left[ r-z_{1}, ... ,r-z_{k}\right]$\;
      $Res\_tmp.append(\left[ r_{1}, ..., r_{k}\right])$\;
      
    }
    $Res_{topk} = find(Res\_tmp, k)$
   
  }
  $Y = find(Res_{topk}, 1) $

  % \vspace{-0.2cm}

\end{algorithm}
% \vspace{-0.2cm}
% -------------------------------------------------------------------------


\subsection{Discriminator and loss function}

The discriminator of the experiments is the same as the discriminator of SMGAN \cite{stylemelgan}. 
The overall function $\mathcal{L}$ can be expressed as:
\begin{equation}
  \begin{split}
    \mathcal{L}= &  \mathcal{L}_{rec}+ \lambda_{feat}\mathcal{L}_{feat}  + \lambda_{adv}\mathcal{L}_{adv} \\
    & +  \lambda_{VQ} \mathcal{L}_{VQ}+ \lambda_{pmsqe} \mathcal{L}_{pmsqe}
  \end{split}
  \end{equation}
$\mathcal{L}_{rec}$ is the multi-scale reconstruction loss, described in \cite{soundstream}. $\mathcal{L}_{feat}$ is the "feature" loss, computed in the feature space defined by the discriminators \cite{soundstream}. $\mathcal{L}_{adv}$ is the adversial loss for the generator. $\mathcal{L}_{VQ}$ is the commitment loss \cite{VQVAE}, which constraints vector quantization. The $\mathcal{L}_{pmsqe}$ is the perceptual loss \cite{pmsqe_loss}, which is designed to be inversely proportional to PESQ \cite{pesq}. In this work, we set $\lambda_{feat}$=100 and $\lambda_{adv}$=$\lambda_{VQ}$ = $\lambda_{pmsqe}$=1. 



==> sections/experiments_xulinping.tex <==
% Experiments
\subsection{Datasets and evaluation metrics}
CBRC was trained on 245 hours of speech from the LibriTTS dataset \cite{libritts} at 16 kHz. To ensure that the model is robust with different audio amplitudes, each segment of 3 seconds was normalized with a maximum peak value of 0.95 and multiplied by a random gain from 0.3 to 1. The model is trained on A100-SXM-80GB with a batch size of 60. The computational complexity of the CBRC is approximately 4.57G Macs and the total number of model parameters is approximately 4.38M. 
In this paper, ViSQOL V3 \cite{visqol}, PESQ \cite{pesq} and POLQA \cite{polqa} are adopted to evaluate the objective quality of CBRC. For subjective test, we used unseen audio samples with a MUSHRA-inspired crowd-sourced method \cite{mush}. 


\subsection{Comparison with other codecs}

To evaluate the audio quality of CBRC with Group-wise($g$=2) and Beam-search($k$=4) RVQ, different codecs were evaluated on a set of 10 clean multilingual speech sequences and the subjective and objective scores are given here. The results in Figure \ref{fig:subjective_score} and Table \ref{tab:different_codecs} show that the audio quality of CBRC at 3kbps outperforms Opus\footnote{https://opus-codec.org} at 12kbps, despite using a quarter of the bitrate.  We also see that CBRC at 3kbps significantly outperforms Lyra-V2\footnote{https://github.com/google/lyra} at 3.2kbps, which demonstrates the superiority of the CBRC architecture. 

% -------------------------------------------------------------------------
% objective scores
\begin{table}[t]
  \caption{Objective scores of different codecs.}
  \label{tab:different_codecs}
  \vspace{-4mm}
  \begin{center}
    \begin{tabular}{lllll}
      Codec      & bitrate & ViSQOL & PESQ  & POLQA \\ \hline
      Opus       & 6kbps   & 2.57   & 2.18  & 3.30  \\
      Opus       & 9kbps   & 3.51   & 3.08  & 3.63  \\
      Lyra-V2       & 3.2kbps   & 3.25   & 1.52  & 3.29  \\
      \textbf{CBRC} & 3kbps   & \textbf{3.52}   & \textbf{2.88}  & \textbf{3.55}  \\ \hline
      Opus       & 12kbps  & 3.91   & 3.81  & 4.04    \\
      \textbf{CBRC} & 6kbps   & \textbf{4.04}    & \textbf{3.57}    & \textbf{3.83}   \\ \hline
      
    \end{tabular}

  \end{center}
  \vspace{-0.5cm}
  \end{table}
% -------------------------------------------------------------------------

% -------------------------------------------------------------------------
% mushra subjective scores
\begin{figure}[t]
  \begin{minipage}[b]{1.0\linewidth}
    \centering
    \centerline{\includegraphics[width=1.0\linewidth]{pics/subjective_score.png}}
  %  \vspace{2.0cm}
  \end{minipage}
  \setlength{\abovecaptionskip}{-0.4cm}
  \caption{Subjective scores for different codecs. Error bars denote 95\% confidence intervals.}
  \label{fig:subjective_score}
  \vspace{-0.3cm}
  
  \end{figure}
% -------------------------------------------------------------------------


\subsection{Ablation of Intra-BRNN}

Several ablation experiments were carried out to evaluate the benefit of Intra-BRNN applied in CBRC. All the models were operated at 6kbps and trained for 300 epochs. Intra-BRNN can be applied in encoder, decoder or both. From the results in Table \ref{tab:dprnn_ablation}, we learn that the Intra-BRNN gets significant improvement with ViSQOL from 3.41 to 4.01 if it is brought in both encoder and decoder. This  demonstrates that Intra-BRNN block could capture temporal information more efficiently than a fully convolutional block. We statistic the frequency of the codeword used in each VQ layer, and calculate the bitrate by entropy coding. The bitrate of the fully convolutional model is about 4.94kbps, while the bitrate of CBRC is 5.13kbps. The bitrate comparison also illustrates that the efficiency of codebook utilization in RVQ can be further improved.

% -------------------------------------------------------------------------
% ablation of Intra-BRNN
\begin{table}[t]
  \caption{Ablation of Intra-BRNN in encoder and decoder. $w/o$ indicates that the fully convolutional network, and $w$ indicates that the interleaved network of 1D-CNN and Intra-BRNN.}
  \label{tab:dprnn_ablation}
  \vspace{-4mm}
  \begin{center}
    \begin{tabular}{c|c|c|c}
      \hline
        & Encoder   & Decoder   & \multirow{2}{*}{ViSQOL} \\
        & Intra-BRNN & Intra-BRNN &                         \\ \hline

        1 & $w/o$        & $w/o$        & 3.41                     \\
        2 & $w/o$       & $w$        & 3.55                    \\
        3 & $w$        & $w/o$        & 3.88                    \\
        4 & $w$       & $w$       &  \textbf{4.01}                      \\\hline

        \end{tabular}

  \end{center}
  \vspace{-0.4cm}
  \end{table}
% -------------------------------------------------------------------------

% -------------------------------------------------------------------------
% comparison of different types of RVQ
\begin{table}[t]
  \caption{Comparison of different types of RVQ.}
  \label{tab:rvq}
  \vspace{-4mm}
  \begin{center}
    \begin{tabular}{c|c}
      Quantizer Type & ViSQOL  \\ \hline
      RVQ            &     3.81     \\
      Group-wise RVQ      &   3.92     \\
      Beam-search  RVQ      &   \textbf{4.02}      \\
      GB-RVQ    &  4.01    \\ \hline          
      \end{tabular}
  \end{center}
  \vspace{-0.7cm}
  \end{table}
  % -------------------------------------------------------------------------




\subsection{Ablation of Group-wise RVQ and Beam-search RVQ}

To demonstrate the effectiveness of the proposed Group-wise RVQ and Beam-search RVQ, ViSQOL scores with different RVQs were evalutated at 6kbps and 300 training epochs. The data in Table \ref{tab:rvq} shows that with the Group-wise($g$=2) and Beam-search($k$=4) algorithm on the basis of RVQ, the ViSQOL scores of CBRC improves  from 3.81 to 3.92 and 4.02, respectively. The Group-wise RVQ improves quantization accuracy and reduces the computational complexity. Beam-search RVQ  slightly increases complexity of the quantization but significantly improves coding quality.  With Group-wise and Beam-search algorithm, the computational complexity of quantizer increases from 0.157G Macs to 0.234G Macs. Considering 4.57G Macs of the model architecture, GB-RVQ improves ViSQOL score from 3.81 to 4.01 with little complexity increase. 






 

